An open-source framework for ExpFinder integrating $N$-gram Vector Space Model and $\mu$CO-HITS

Finding experts drives successful collaborations and high-quality product development in academic and research domains. To contribute to the expert finding research community, we have developed ExpFinder which is a novel ensemble model for expert finding by integrating an $N$-gram vector space model ($n$VSM) and a graph-based model ($\mu$CO-HITS). This paper provides descriptions of ExpFinder's architecture, key components, functionalities, and illustrative examples. ExpFinder is an effective and competitive model for expert finding, significantly outperforming a number of expert finding models.

==> ExpFinder_ ElsevierSI/extension.tex <==
\section{Extension}
\begin{figure}[!h]
    \centering
    \includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=150pt]{figures/extensions.pdf}
    \caption{A graph showing the use of ExpFinder's output in other expert finding models} 
    \label{fig:extensions}
\end{figure}

With the blueprint in Section \ref{sec:func} and illustrative examples in Section \ref{sec:example}, we have observed that the output of ExpFinder can potentially be used in other expert finding models, as shown in Figure \ref{fig:extensions}. In BMExpert \cite{Wang2015} as one DLM, DTM can be an input for two factors such as relevance of documents to given topics and importance of documents, and EDM shows associations between experts and documents. Thus, Figure \ref{fig:extensions} shows the directed edge from DTM and EDM to BMExpert. Similarly, WISER \cite{WISER2019} is another DLM that takes an advantage of ExpFinder's output. In this model, DTM can be an input in the calculation of BM25 \cite{BM25} which further integrates with EDM to interpret the importance of experts' documents given a topic. On the other hand, in GM, Author-Document-Topic (ADT) model \cite{Gollapalli2013} can use EDM to construct an undirected graph showing connections between author and document layers and DTopM to construct an undirected, weighted graph showing connections between document and topic layers. 

==> ExpFinder_ ElsevierSI/functionality.tex <==
\section{Functionality} \label{sec:func}

ExpFinder is implemented in Python (version $\geq$ 3.6) with open-source libraries such as \texttt{pandas}, \texttt{NumPy}, \texttt{scikit-learn}, \texttt{SciPy},  \texttt{nltk}, and \texttt{networkx}. In this section, we present its architecture, key components, and their functionalities. The architecture of ExpFinder is presented in Figure \ref{fig:func_graph} that consists of four key steps with the corresponding functions and their functional dependencies:

\begin{figure*}[!t]
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=350pt]{figures/dep_func.pdf}
\caption{The architecture and functional workflow of ExpFinder: blue labels indicate module names of ExpFinder, and `Output Relation' maps the functional component to the corresponding processing step.}
\label{fig:func_graph}
\end{figure*}

\begin{enumerate}
    \item \textbf{Step 1 - Extract tokens and topics}: Given an expertise source $\mc{D}$ (e.g., scientific publications) of experts $\mc{X}$, we extract expertise topics by using  \texttt{tokenise\_doc()} in \textbf{extractor.py}. We assume that expertise topics are represented in the forms of noun phrases. For each document $d\in \mc{D}$, the function splits it into sentences. Then, for each sentence, the function removes stopwords, assigns a part of speech (POS) to each word, merges the inflected forms of a word (i.e., the lemmatisation process, for example, `patients' is lemmatised to `patient'), and extracts single-word terms (called \textit{tokens}) and topics with a given linguistic pattern. In addition, we use a regular expression (\texttt{regex}) in Python to construct a linguistic pattern based on POS that is further used for extracting four different types of topics as shown in Figure \ref{fig:regex}. 
    \begin{figure}[!h]
    \centering
    \includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=250pt]{figures/regex.pdf}
    \caption{The Python regular expression of a linguistic pattern for extracting topics in a single document} 
    \label{fig:regex}
    \end{figure}
    Note that we use \texttt{nltk} for performing this process. The output of this step is the list of the tokens and the list of topics for each document $d \in \mc{D}$. The set of the all tokens is denoted as $\mc{W}$, and the set of the all topics is denoted as $\mc{T}$.

    \item \textbf{Step 2 - Estimate the weights of experts and documents given topics in $n$VSM}: The process includes four main steps with the corresponding functions in \textbf{generator.py}:
    \begin{enumerate}
        \item We use \texttt{generate\_tf()} to estimate the term frequencies (TFs) of $\mc{W}$ in each document $d \in \mc{D}$. For this estimation, we use \texttt{CountVectoerizer} in \texttt{scikit-learn}. The output of this function is the $|\mc{D}| \times |\mc{W}|$ Document-Token matrix (\textbf{DTM}) where each entry contains the TF of $w \in \mc{W}$ in $d$.
        
        \item We use  \texttt{generate\_dp\_matrix()} to estimate the weights of documents given $\mc{T}$ in $n$VSM \cite{kang2021expfinder}. The function estimates $n$TFIDF of each topic $t \in \mc{T}$ by integrating the $n$TF weighting and  the $n$IDF weighting. Intuitively, $n$TF estimates the frequency of $t$ by averaging TFs of tokens in $t$ where TF of each token is stored in \textbf{DTM}. In addition, $n$IDF \cite{nidf:2017} is the $N$-gram IDF weighting method that estimates the log-IDF, $\log\frac{|\mc{D}| \times df(t) + 1}{df(w_{1} \land w_{2} \land \ldots \land w_{n})^{2} + 1} +1$, of $t$ where $w_{1}, \ldots, w_{n}$ are $n$-constituent terms in $t$. The output of this step is the $|\mc{D}| \times |\mc{T}|$ Document-Phrase matrix (\textbf{DPM}) where each entry contains the $n$TFIDF weight of $t$ in $d$.
        
        \item Given $\mc{D}$, we use  \texttt{genenerate\_ed\_matrix()} to generate the $|\mc{X}| \times |\mc{D}|$ Expert-Document matrix (\textbf{EDM}) where each entry shows a binary relationship between $x \in \mc{X}$ and $d$ (e.g., 1 indicates that $x$ has the authorship on $d$, and 0 otherwise). 
        
        
        \item We use  \texttt{generate\_pr\_matrix()} to estimate the weights of experts $\mc{X}$ and documents $\mc{D}$ given each topic $t \in \mc{T}$ in $n$VSM \cite{kang2021expfinder}. The weights of $\mc{X}$ are estimated by calculating matrix multiplication of $\textbf{EDM}^{|\mc{X}| \times |\mc{D}|}$ and $\textbf{DPM}^{|\mc{D}| \times |\mc{T}|}$ (e.g., \textbf{ETopM} \texttt{= numpy.matmul(}\textbf{EDM}, \textbf{DPM}\texttt{)} in Python). The output is the $|\mc{X}| \times |\mc{T}|$ Expert-Topic matrix (\textbf{ETopM}) where each entry contains the topic-sensitive weight of $x$ given $t$. The weights of $\mc{D}$ are represented by \textbf{DPM}.  Now, we denote \textbf{DPM} as the $|\mc{D}| \times |\mc{T}|$ Document-Topic matrix (\textbf{DTopM}) where each entry shows the topic-sensitive weight of $d$ given $t$. It is worth noting that \textbf{DPM} can be integrated with another factor (e.g., the average document frequencies of $\mc{T}$) to obtain different weights for \textbf{DTopM}. However, in our approach, we set $\textbf{DTopM} = \textbf{DPM}$.
        
    \end{enumerate}

    \item \textbf{Step 3 - Construct ECG}. We use  \texttt{generate\_ecg()} in \textbf{generator.py} to handle this step. The function receives $\mc{D}$ and builds an ECG using \texttt{DiGraph} in \texttt{networkx} to present a \textit{directed, weighted bipartite graph} that has expert nodes $V_{x}$ and document nodes $V_{d}$. The set of nodes in the graph is denoted as $V$ such that $V = V_x \cup V_d$. A directed edge points from a document node $v_{d} \in V_{d}$ to an expert node $v_{x} \in V_{x}$ if $x$ has published $d$. In this step, we also use \texttt{generate\_ed\_vector()} in \textbf{generator.py} to generate a $|V| \times 1$ Expert-Count vector ($\boldsymbol{c_{x}}$) and a $|V| \times 1$ Document-Count ($\boldsymbol{c_{d}}$) vector based on ECG. These vectors are used for the estimation of $\mu$CO-HITS in \textbf{Step 4}.
    
 
    
    \item \textbf{Step 4 - Reinforce expert weights using $\mu$CO-HITS}. We use \texttt{run\_expfinder()} in \textbf{trainer.py} to handle this step. The function receives \textbf{ETopM}, \textbf{DTopM}, ECG, $\boldsymbol{c_{x}}$ and $\boldsymbol{c_{d}}$, generated in \textbf{(Steps 2 and 3)} as parameters, and reinforces the estimation of expert weights given topics by integrating $n$VSM and $\mu$CO-HITS \cite{kang2021expfinder}. For each $t \in \mc{T}$, we perform the three steps:
    
    \begin{enumerate}
        \item \textbf{Generate the adjacency matrix of nodes and its transpose} - Given the ECG, we use  \texttt{to\_matrix()} in \texttt{networkx} to generate the $|V| \times |V|$ adjacency matrix of the graph $\textbf{M}$, and also construct its  transpose matrix $\textbf{M}^{\top}$. These matrices are required in the initialisation for running the $\mu$CO-HITS algorithm.
        
        \item \textbf{Normalise the weights of experts and documents given a topic} - We get topic-sensitive weights of $\mc{X}$ and $\mc{D}$ given $t$ from \textbf{ETopM} and \textbf{DTopM}, respectively. The output of this includes the $|\mc{X}| \times 1$ Expert-Topic ($\boldsymbol{\alpha_{x}}$) and $|\mc{D}| \times 1$ Document-Topic ($\boldsymbol{\alpha_{d}}$) vectors where each entry shows the topic-sensitive weight of an expert and a document given $t$, respectively. Then, we normalise these vectors using L2 normalisation to scale their squares sum to 1 as the initialisation for running the $\mu$CO-HITS algorithm \cite{kleinberg1999authoritative}.
        
        \item \textbf{Reinforce expert weights given a topic} - We integrate $n$VSM and $\mu$CO-HITS through $k$ iterations to reinforce expert weights given $t$. $\mu$CO-HITS is the extension of the CO-HITS algorithm \cite{Hongbo2009} which contains two main properties such as \textit{average authorities} $\boldsymbol{a}$ and \textit{average hubs} $\boldsymbol{h}$ which show importance of $\mc{X}$ and $\mc{D}$, respectively, based on the ECG. In addition, these properties can be defined as \cite{kang2021expfinder}:
        \begin{align}
            \boldsymbol{a}(\mc{X}; t)^{k} &= (1 - \lambda_{x}) \boldsymbol{a}(\mc{X}; t)^{k - 1} + \lambda_{x} \left( \frac{ \textbf{M}^{\top} \boldsymbol{\cdot} \boldsymbol{h}(\mc{D}; t)^{k - 1} }{ \boldsymbol{c_{d}} } \right) \\
            \boldsymbol{h}(\mc{D}; t)^{k} &= (1 - \lambda_{d}) \boldsymbol{h}(\mc{D}; t)^{k - 1} + \lambda_{d} \left( \frac{ \textbf{M} \boldsymbol{\cdot} \boldsymbol{a}(\mc{X}; t)^{k} }{ \boldsymbol{c_{x}} }  \right)
        \end{align}
        where
        \begin{itemize}
            \item $\boldsymbol{a}(\mc{X}; t)^{k}$ and $\boldsymbol{h}(\mc{D}; t)^{k}$ are  $|V| \times 1$ vectors which contain the reinforced expert weights and reinforced document weights, respectively, given $t$ at $k^{\text{th}}$ iteration. As the initial weights of these vectors, we use the topic-sensitive weights of experts and documents estimated in $n$VSM. Thus, $\boldsymbol{a}(\mc{X}; t)^{0} = \boldsymbol{\alpha_{x}}$ and $\boldsymbol{h}(\mc{D}; t)^{0} = \boldsymbol{\alpha_{d}}$. By doing so, we integrate $n$VSM with $\mu$CO-HITS. Note that $\boldsymbol{a}(\mc{X}; t)^{0}$ is a $|\mc{X}| \times 1 $ vector, and $\boldsymbol{h}(\mc{D}; t)^{0}$ is a $|\mc{D}| \times 1$ vector. However, for easily implementing the HITS algorithm, we have transformed the dimension of these vectors into $|V| \times 1$ vectors where  additional entries hold the value of 0.
            
            \item $\lambda_{x} \in [0, 1]$ and $\lambda_{d} \in [0, 1]$ are \textit{parameters} for expert and document, respectively. These are used to control the impact of topic-sensitive weights on $\boldsymbol{a}$ and $\boldsymbol{h}$, respectively. Assigning lower values indicates the higher impact of topic-sensitive weights on $\boldsymbol{a}$ and $\boldsymbol{h}$.
            
            \item $\left( \frac{ \textbf{M}^{\top} \boldsymbol{\cdot} \boldsymbol{h}(\mc{D}; t)^{k - 1} }{ \boldsymbol{c_{d}} } \right)$ is the calculation for the \textit{average authorities}. The numerator performs  matrix multiplication between the $|V| \times |V|$ adjacency matrix $\textbf{M}^{\top}$ and the $|V| \times 1$ $\boldsymbol{h}$. The denominator is a $|V| \times 1$ counted vector $\boldsymbol{c_{d}}$ generated in \textbf{Step 3}. To calculate this in Python, we simply apply \texttt{numpy.matmul(}$\textbf{M}^{\top}$, $\boldsymbol{h}(\mc{D}; t)^{k - 1}$\texttt{)/}$\boldsymbol{c_{d}}$.
            
            \item $\left( \frac{ \textbf{M} \boldsymbol{\cdot} \boldsymbol{a}(\mc{X}; t)^{k} }{ \boldsymbol{c_{x}} }  \right)$ is the calculation for the \textit{average hubs}. The numerator performs  matrix multiplication between the $|V| \times |V|$ adjacency matrix $\textbf{M}$ and the $|V| \times 1$ $\boldsymbol{a}$. The denominator is a $|V| \times 1$ counted vector $\boldsymbol{c_{x}}$ generated in \textbf{Step 3}. To calculate this in Python, we simply apply \texttt{numpy.matmul(}$\textbf{M}$, $\boldsymbol{a}(\mc{X}; t)^{k}$\texttt{)/}$\boldsymbol{c_{x}}$.
        \end{itemize}
        After computing $\boldsymbol{a}$ and $\boldsymbol{h}$ at $k^{\text{th}}$ iteration, we apply L2 normalisation to both $\boldsymbol{a}$ and $\boldsymbol{h}$. 
        We use the obtained $\boldsymbol{a}(\mc{X}; t)$ after the final iteration to construct the $|\mc{X}| \times |\mc{T}|$ Expert-Topic matrix (\textbf{RETopM}) where each entry contains the reinforced weight of $x$ given $t$.
        
    \end{enumerate}

\end{enumerate}

==> ExpFinder_ ElsevierSI/impact.tex <==
\section{Impact and Conclusion} \label{sec:impact}
With the growth of expertise digital sources, expert finding is a crucial task that has significantly helped people to seek the services and guidance of an expert \cite{gonccalves2019automated}. ExpFinder is an ensemble model for expert finding that integrates $n$VSM with $\mu$CO-HITS to enhance the capability for expert finding over existing DLM, VSM and GM approaches. To our best knowledge, ExpFinder is the first attempt to provide the implementation of $n$VSM and $\mu$CO-HITS for expert finding.

The implementation of ExpFinder also provides functionalities that can be potentially useful for implementing other expert finding models. For example, our tokenisation module for extracting noun phrases using a linguistic pattern based on a part of speech (POS) can be easily customised based on researchers' purposes. The modules for building the presented Expert-Document matrix (\textbf{EDM}), Expert-Topic matrix (\textbf{ETopM}), and Document-Topic matrix (\textbf{DTopM}) can be usefully leveraged to represent relationships between experts and documents, experts and topics, and documents and topics. These relationships can be used to represent a collective information among experts, documents and topics and used to implement other graph-based expert finding models such as an author-document-topic (ADT) graph \cite{Gollapalli2013} and an expert-expert graph via topics.  

We highlight that ExpFinder is a state-of-the-art model, substantially outperforming the following widely known and latest models for expert finding: {document language models} \cite{Balog2009}, probabilistic-based expert finding model \cite{WISER2019}), {graph-based models} \cite{Hongbo2009, Gollapalli2013, Daniel2015}. Thus, the ones who want to extend ExpFinder can harness our implementation for further improvement of ExpFinder.

We presented the architecture and implementation detail of ExpFinder with an illustrative example. This would help researchers and practitioners to better understand how ExpFinder is designed and implemented with its core functionalities.

==> ExpFinder_ ElsevierSI/intro.tex <==
\section{Introduction}

\begin{figure*}[!t]
    \centering
    \includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=350pt]{figures/intro_method.pdf}
    \caption{The overview of ExpFinder} 
    \label{fig:intro_method}
\end{figure*}

Identifying experts given a query topic, known as \textit{expert finding}, is a crucial task that accelerates rapid team formation for research innovations or business growth. Existing expert finding models can be classified into three categories such as \textit{vector space models} (VSM) \cite{riahi2012finding, chuang2014combining}, \textit{document language models} (DLM) \cite{Balog2009, Wang2015, WISER2019}, or \textit{graph-based models} (GM) \cite{Hongbo2009, Gollapalli2013, Daniel2015}. ExpFinder \cite{kang2021expfinder} is an ensemble model for expert finding which integrates a novel $N$-gram VSM ($n$VSM) with a GM ($\mu$CO-HITS)-a variant of the generalised CO-HITS algorithm \cite{Hongbo2009}. 

As seen in Figure \ref{fig:intro_method}, ExpFinder has $n$VSM, a vector space model, as a key component that estimates the weight of an expert and a document given a topic by leveraging the Inverse Document Frequency (IDF) weighting~\cite{nidf:2017} for $N$-gram words (simply $N$-grams). Another key component in ExpFinder is $\mu$CO-HITS that is used to reinforce the weights of experts and documents given a topic in $n$VSM using an Expert Collaboration Graph (ECG) that is a certain form of an expert social network. The output of ExpFinder is the reinforced weights of experts given topics. 

ExpFinder is designed and developed to improve the performance for expert finding. In this paper, we highlight two main contributions to the expert finding community. First, we provide a comprehensive implementation detail of all steps taken in ExpFinder. It could also be used as an implementation guideline for developing various DLM-, VSM- and GM-based expert finding approaches. Second, we illustrate how ExpFinder works with a simple example, thus researchers and practitioners can easily understand ExpFinder's design and implementation.

This paper is organised as follows. Section \ref{sec:func} describes ExpFinder's architecture and functionalities. Section \ref{sec:example} demonstrates the procedural steps in ExpFinder. Section \ref{sec:impact} provides the impact and conclusion of ExpFinder.



==> extension.tex <==
\section{Extension}
\begin{figure}[!h]
    \centering
    \includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=150pt]{figures/extensions.pdf}
    \caption{A graph showing the use of ExpFinder's output in other expert finding models} 
    \label{fig:extensions}
\end{figure}

With the blueprint in Section \ref{sec:func} and illustrative examples in Section \ref{sec:example}, we have observed that the output of ExpFinder can potentially be used in other expert finding models, as shown in Figure \ref{fig:extensions}. In BMExpert \cite{Wang2015} as one DLM, DTM can be an input for two factors such as relevance of documents to given topics and importance of documents, and EDM shows associations between experts and documents. Thus, Figure \ref{fig:extensions} shows the directed edge from DTM and EDM to BMExpert. Similarly, WISER \cite{WISER2019} is another DLM that takes an advantage of ExpFinder's output. In this model, DTM can be an input in the calculation of BM25 \cite{BM25} which further integrates with EDM to interpret the importance of experts' documents given a topic. On the other hand, in GM, Author-Document-Topic (ADT) model \cite{Gollapalli2013} can use EDM to construct an undirected graph showing connections between author and document layers and DTopM to construct an undirected, weighted graph showing connections between document and topic layers. 
